Automatic Configuration for Optimal Communication Scheduling in DNN Training

ByteScheduler partitions and rearranges tensor transmissions to improve the communication efficiency of distributed Deep Neural Network (DNN) training. The configuration of hyper-parameters (i.e., the partition size and the credit size) is critical to the effectiveness of partitioning and rearrangement. Currently, ByteScheduler adopts Bayesian Optimization (BO) to find the optimal configuration for the hyper-parameters beforehand. In practice, however, various runtime factors (e.g., worker node status and network conditions) change over time, making the statically-determined one-shot configuration result suboptimal for real-world DNN training. To address this problem, we present a real-time configuration method (called AutoByte) that automatically and timely searches the optimal hyper-parameters as the training systems dynamically change. AutoByte extends the ByteScheduler framework with a meta-network, which takes the system's runtime statistics as its input and outputs predictions for speedups under specific configurations. Evaluation results on various DNN models show that AutoByte can dynamically tune the hyper-parameters with low resource usage, and deliver up to 33.2\% higher performance than the best static configuration in ByteScheduler.

==> sections/20-motivation_bak.tex <==
\section{Background and Motivation}
\label{sec:background}

In this section, we first introduce the background of GNNs and then demonstrate scalability issues in distributed GNN training from prior work through analysis and experiments.

\subsection{Graph Neural Networks (GNNs)} 
\label{subsec:background_gnn}

GNNs are trained on graph-structured data (i.e., nodes and links) to learn node representations \cite{gcn, graphsage, gat, gin}. 

Figure \ref{figure:gnn} shows the process of performing GNN computation on a data sample (a node from the input graph) in one single GNN layer. The GNN layer first aggregates the node's neighbor nodes' embedding calculated from the preceding GNN layer, and then it applies standard DNN operations such as matrix multiplication to the aggregation result, and finally outputs a new embedding for that node.

To train a GNN, in the forward propagation, the above computation repeats when a node travels through each GNN layer. In the last layer, GNN outputs a representation vector which is used to generate a loss. With the loss, gradients are then calculated from the last layer to the first layer in the backward propagation. Formally, the computation process of GNN is as follows:

\begin{align*}
    a_v^{(k)} \quad &= \quad \i{Aggregate}^{(k)}(\{h_{u}^{(k-1)}\ |\ u \in \mathcal{N}(v)\}) \\
    h_v^{(k)} \quad &= \quad \i{Update}^{(k)}(h_{v}^{(k-1)}, a_{v}^{(k)})
\end{align*}

In the equations above, $h_v^{(k)}$ denotes the node embedding of node $v$ in the $k^{th}$ GNN layer.  $\mathcal{N}(v)$ denotes neighbors of $v$. For each node $v$ in layer $k$, \i{Aggregate} first outputs $a_v^{(k)}$ by gathering the embeddings of its neighbors $h_{u \in \mathcal{N}(v)}^{(k-1)}$ with an accumulation function such as mean or sum, then \i{Update} computes the node's new embedding from its previous embedding $h_v^{(k-1)}$ and aggregation result $a_v^{(k)}$. 

The embeddings from the last layer $h_v^K$ capture information for all neighbors within $K$ hops of $v$, and will be passed to end tasks to generate a loss, thus the model parameters of GNN can be trained end-to-end.

Note that GNN’s propagation between consecutive layers is not only over the same data sample (as in DNN), but also across different data samples (because of neighborhood aggregation operations), and these cross-data-sample propagation paths create computation dependencies between data samples.

%\begin{figure}
%\includegraphics[width=\linewidth]{figures/illustration-gnn-computation.pdf}
%\caption{\b{Computation of one node in layer $K$ by first aggregating its neighbors’ embeddings from previous layer $K-1$, then applying NN operations. }}
%\label{figure:gnn}
%\end{figure}

\subsection{Distributed GNN Training} 
\label{subsec:motivation}

When taking real-world graphs with tens of millions of nodes and billions of links as input, GNN training is time-consuming and cannot fit into single GPU memory. 

Unlike DNNs which can be trained in a distributed manner on independent data partitions, performing GNN computation on one node depends on a huge number of other nodes. As discussed in $\S$\ref{subsec:background_gnn}, computation for a single node's embedding in layer $K$ requires the node's neighbor nodes' embeddings from layer $K$-$1$, which again requires their neighbors' embeddings from layer $K$-$2$ recursively until layer $1$. The amount of data needed grows exponentially with the number of GNN layers, making GNN training both compute-intensive and network-intensive. Some previous works have proposed techniques to improve the efficiency of GNN training on large graphs, and we summarize them as follows.

\b{Neighbor Sampling in GNN Models.} Some GNN models use neighbor sampling strategies that down-sample nodes' neighbors in the neighborhood aggregation operation to reduce calculation cost \cite{graphsage, webscale, fastgcn,zeng2019graphsaint}, bringing speedup to the training process. However, as observed in previous works \cite{roc, huang2021gnn}, these techniques come with the cost of model accuracy loss.
As a typical example, Hamilton et al. \cite{graphsage} proposed a GNN design that samples and aggregates only a small number (between 10 to 25) of neighbors for each node, even when that node may have thousands of neighbors.
Table shows the performance comparison between sampling-based and sampling-free GNN models. Sampling-free GNNs demonstrate improved accuracy compared to the sampling-based models. Moreover, Graph Convolution Networks (GCNs) with deeper model architectures, which can be trained efficiently with \sys, demonstrate better accuracies comparing to others.
In $\S$, we show that \sys can efficiently train GNN models on large graphs without sampling neighbors, achieving better accuracy with comparable throughput of training sample-based models in DGL.


\b{Data Parallelism with Graph Partitioning.} Many existing GNN frameworks \cite{distdgl, aligraph, neugraph, roc} leverage data parallelism by partitioning the input graph and sending each partition to a different worker, where each worker can simultaneously train GNN over its assigned graph partition. However, because of the neighbor aggregation operation, there are still inter-layer computation dependencies between cross-partition neighboring data samples (as shown in Figure \ref{figure:gnn}), making graph partitions dependent on each other in the parallel GNN training process. 

%\begin{figure}
%\includegraphics[width=\linewidth]{figures/motivation.pdf}
%\caption{\b{Scalability of previous GNN systems when training GraphSAGE without neighbor sampling on reddit dataset on a 16-node cluster. Data is rescaled based on each system's training throughput (epoch/s) on a single worker.}}
%\label{figure:motivation}
%\end{figure}

%\input{sections/components/table-motivation}


These computation dependencies, which are determined by the input graph structure, are usually large and complex when training GNNs over real-world graphs. We have observed two schemes of handling the dependencies in previous GNN systems:
(1) layer-wise communication barriers: because the computation dependencies only exist between consecutive GNN layers, NeuGraph \cite{neugraph} implements layer-wise communication barriers for global synchronization of intermediate results. This method introduces system overhead due to the collective communication cost and potential stragglers from unbalanced workload. 
(2) cross-partition multi-hop neighbor replication: widely adopted in DGL \cite{distdgl}, AliGraph \cite{aligraph} and Roc \cite{roc}, this method replicates all out-of-partition neighboring node data to a worker, so that the worker can train GNN over a graph partition independently. It causes duplicate computation and communication among all workers, because the same data may be loaded and used for computation in all $P$ workers, causing duplicate workload for at most $P-1$ times. Moreover, the amount of replicated data grows exponentially to the number of GNN layers.

Our evaluations confirm the analysis above. Figure \ref{figure:motivation} shows the speedup of training throughput on the Reddit dataset without neighbor sampling techniques. As shown in the figure, when the number of workers increases, the scalability of both systems is far from linear, and when the number of workers reaches 16, we start to observe zero returns in training speedup. 

\subsection{Model Explanation} 
\label{subsec:explanation}
